Temporal logic control of general Markov decision processes by approximate policy refinement

The formal verification and controller synthesis for Markov decision processes that evolve over uncountable state spaces are computationally hard and thus generally rely on the use of approximations. In this work, we consider the correct-by-design control of general Markov decision processes (gMDPs) with respect to temporal logic properties by leveraging approximate probabilistic relations between the original model and its abstraction. We newly work with a robust satisfaction for the construction and verification of control strategies, which allows for both deviations in the outputs of the gMDPs and in the probabilistic transitions. The computation is done over the reduced or abstracted models, such that when a property is robustly satisfied on the abstract model, it is also satisfied on the original model with respect to a refined control strategy.

==> fig04.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmin=1,
xmax=11,
ymin=0,
ymax=3,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, draw=none, mark=x, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
1	2.65\\
2	1.95\\
3	1.45\\
4	1.35\\
5	1.25\\
6	1.05\\
7	0.75\\
8	0.649999999999999\\
9	0.45\\
10	0.649999999999999\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
1	2.45\\
2	2.08281825883856\\
3	1.72297166354556\\
4	1.43203695709684\\
5	1.21690498767597\\
6	1.05454638058171\\
7	0.880512997649619\\
8	0.689425568595503\\
9	0.533871365035334\\
10	0.414391332403024\\
11	0.391748675132592\\
};
\addplot [color=mycolor3, draw=none, mark=x, mark options={solid, mycolor3}, forget plot]
  table[row sep=crcr]{%
1	2.65\\
2	1.95\\
3	1.45\\
4	1.25\\
5	1.05\\
6	0.75\\
7	0.55\\
8	0.55\\
9	0.55\\
10	0.45\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
1	2.45\\
2	2.0871113747558\\
3	1.7428081605892\\
4	1.43212362636695\\
5	1.19378301181628\\
6	0.955399219287496\\
7	0.7311315249561\\
8	0.546350199258822\\
9	0.439466169410851\\
10	0.347023167036659\\
11	0.282554458630428\\
};
\addplot [color=mycolor5, draw=none, mark=x, mark options={solid, mycolor5}, forget plot]
  table[row sep=crcr]{%
1	2.65\\
2	1.95\\
3	1.45\\
4	1.35\\
5	1.05\\
6	0.95\\
7	0.95\\
8	0.75\\
9	0.75\\
10	0.55\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
1	2.45\\
2	2.08437242029748\\
3	1.72964250424555\\
4	1.43256266099907\\
5	1.21546678473743\\
6	0.992270428898916\\
7	0.839742570952465\\
8	0.72036722767742\\
9	0.600287536685836\\
10	0.50011691129157\\
11	0.379700889442169\\
};
\addplot [color=mycolor7, draw=none, mark=x, mark options={solid, mycolor7}, forget plot]
  table[row sep=crcr]{%
1	2.65\\
2	1.95\\
3	1.45\\
4	1.45\\
5	1.15\\
6	1.05\\
7	0.850000000000001\\
8	0.55\\
9	0.55\\
10	0.350000000000001\\
};
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
1	2.45\\
2	2.08325216234967\\
3	1.72644664053003\\
4	1.44940682976872\\
5	1.26307576843685\\
6	1.04449841608698\\
7	0.871148580223421\\
8	0.710470267671952\\
9	0.530648338704551\\
10	0.398506689964389\\
11	0.27030802594444\\
};
\addplot [color=mycolor2, draw=none, mark=x, mark options={solid, mycolor2}, forget plot]
  table[row sep=crcr]{%
1	2.65\\
2	1.85\\
3	1.35\\
4	1.05\\
5	0.95\\
6	0.75\\
7	0.75\\
8	0.75\\
9	0.850000000000001\\
10	0.75\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
1	2.45\\
2	2.0772947215596\\
3	1.68891743467978\\
4	1.3717482384539\\
5	1.10213105092041\\
6	0.89691729369732\\
7	0.716580065595192\\
8	0.597768286705844\\
9	0.523060979159613\\
10	0.487065777871116\\
11	0.405949067969639\\
};
\addplot [color=mycolor4, draw=none, mark=x, mark options={solid, mycolor4}, forget plot]
  table[row sep=crcr]{%
1	2.65\\
2	1.85\\
3	1.45\\
4	1.15\\
5	1.05\\
6	0.95\\
7	0.95\\
8	0.649999999999999\\
9	0.55\\
10	0.45\\
};
\addplot [color=mycolor5, forget plot]
  table[row sep=crcr]{%
1	2.45\\
2	2.07758538156955\\
3	1.69809006231344\\
4	1.41307036584877\\
5	1.13738862532075\\
6	0.952014365546549\\
7	0.797246278063067\\
8	0.688231149487747\\
9	0.524584574827064\\
10	0.410446498436523\\
11	0.315811946468197\\
};
\addplot [color=mycolor6, draw=none, mark=x, mark options={solid, mycolor6}, forget plot]
  table[row sep=crcr]{%
1	2.65\\
2	2.05\\
3	1.55\\
4	1.25\\
5	0.95\\
6	0.850000000000001\\
7	0.850000000000001\\
8	0.75\\
9	0.75\\
10	0.45\\
};
\addplot [color=mycolor7, forget plot]
  table[row sep=crcr]{%
1	2.45\\
2	2.08757422741894\\
3	1.7549242426729\\
4	1.47743988099213\\
5	1.19200132120817\\
6	0.959745423464698\\
7	0.780160877253685\\
8	0.665133984079329\\
9	0.550736642387298\\
10	0.463973836593935\\
11	0.330710595483775\\
};
\addplot [color=mycolor1, draw=none, mark=x, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
1	2.65\\
2	1.85\\
3	1.15\\
4	1.05\\
5	0.95\\
6	0.850000000000001\\
7	0.649999999999999\\
8	0.649999999999999\\
9	0.649999999999999\\
10	0.55\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
1	2.45\\
2	2.07768139490263\\
3	1.68104374922527\\
4	1.32335770020432\\
5	1.07622543290764\\
6	0.879841144887135\\
7	0.70973102546008\\
8	0.547717930397934\\
9	0.470549027258106\\
10	0.398957098087294\\
11	0.326394933925277\\
};
\addplot [color=mycolor3, draw=none, mark=x, mark options={solid, mycolor3}, forget plot]
  table[row sep=crcr]{%
1	2.65\\
2	1.95\\
3	1.25\\
4	0.95\\
5	0.75\\
6	0.649999999999999\\
7	0.45\\
8	0.350000000000001\\
9	0.25\\
10	0.350000000000001\\
};
\addplot [color=mycolor4, forget plot]
  table[row sep=crcr]{%
1	2.45\\
2	2.08105094144378\\
3	1.69914927389061\\
4	1.33438418443958\\
5	1.05752257857596\\
6	0.818949754117422\\
7	0.615968525378736\\
8	0.446628460712029\\
9	0.314315876454544\\
10	0.185747938625319\\
11	0.153017814510057\\
};
\addplot [color=mycolor5, draw=none, mark=x, mark options={solid, mycolor5}, forget plot]
  table[row sep=crcr]{%
1	2.65\\
2	1.95\\
3	1.35\\
4	1.05\\
5	1.05\\
6	0.850000000000001\\
7	0.75\\
8	0.75\\
9	0.649999999999999\\
10	0.55\\
};
\addplot [color=mycolor6, forget plot]
  table[row sep=crcr]{%
1	2.45\\
2	2.08250274694372\\
3	1.71766155327182\\
4	1.39866695369378\\
5	1.12459444091449\\
6	0.939007741931164\\
7	0.765132051656333\\
8	0.615380404070769\\
9	0.5375845282806\\
10	0.442918007569914\\
11	0.351034337112777\\
};
\end{axis}
\end{tikzpicture}%
